Graph Embedded Pose Clustering for Anomaly Detection

We propose a new method for anomaly detection of human actions. Our method works directly on human pose graphs that can be computed from an input video sequence. This makes the analysis independent of nuisance parameters such as viewpoint or illumination. We map these graphs to a latent space and cluster them. Each action is then represented by its soft-assignment to each of the clusters. This gives a kind of "bag of words" representation to the data, where every action is represented by its similarity to a group of base action-words. Then, we use a Dirichlet process based mixture, that is useful for handling proportional data such as our soft-assignment vectors, to determine if an action is normal or not. We evaluate our method on two types of data sets. The first is a fine-grained anomaly detection data set (e.g. ShanghaiTech) where we wish to detect unusual variations of some action. The second is a coarse-grained anomaly detection data set (e.g., a Kinetics-based data set) where few actions are considered normal, and every other action should be considered abnormal. Extensive experiments on the benchmarks show that our method performs considerably better than other state of the art methods.

==> drawings/tex/fail_cases_kin.tex <==
\begin{figure}
\begin{center}
\begin{tabular}{@{\hskip 0in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.06in}@{\hskip 0in}}
\includegraphics[width=0.3\linewidth]{drawings/dataset_imgs/w_pose/lunge_wpose1.png} & 
\includegraphics[width=0.3\linewidth]{drawings/dataset_imgs/w_pose/pushup2_wpose1.png}  &
\includegraphics[width=0.3\linewidth]{drawings/dataset_imgs/w_pose/lunge_fail_border_wpose1.png} \\ 
\includegraphics[width=0.3\linewidth]{drawings/dataset_imgs/w_pose/situp_wpose1.png} & 
\includegraphics[width=0.3\linewidth]{drawings/dataset_imgs/w_pose/squat3_wpose1.png} & 
\includegraphics[width=0.3\linewidth]{drawings/dataset_imgs/w_pose/taichi_fail_border_wpose1.png} \\

\multicolumn{1}{c}{(a)} & \multicolumn{1}{c}{(b)} & \multicolumn{1}{c}{(c)}  \vspace{-0.25cm}\\
% (a) & (b) & (c) \vspace{-0.30cm}
\end{tabular}
\end{center}
\caption{{\small \textbf{Failure Cases, \textit{Kinetics-250}:} Frames overlayed with extracted poses from ``Gym'' split: Columns (a)-(b) depict dataset classes ``Lunge'', ``Push ups'', ``Situp'' and ``Squat''. Column (c) depicts failure cases; Top: a ``normal'' {\it lunge} sequence, mislabeled as ``abnormal'' in a clip where the instructor remains static for most of the time. Bottom: an ``abnormal'' {\it Tai-chi} clip labeled ``normal'' when the instructor demonstrates a push up like hand movement.}
\vspace{-0.2cm}}
\label{fig:fail_cases}
\end{figure}

==> drawings/tex/failure_cases_fig_2dataset.tex <==
\begin{figure}
\begin{center}
\begin{tabular}{@{\hskip 0in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.07in}c@{\hskip 0.05in}c@{\hskip 0.01in}@{\hskip 0in}}
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/lunge1.png} & 
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/pullups1_resized.png} & 
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/push_ups_resized.png} & 
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/situp_resized.png} & 
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/squat_resized.png} & 
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/lunge1.png} \\
\hline \vspace{0.1cm}
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/lunge1.png} & 
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/pullups1_resized.png} & 
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/push_ups_resized.png} & 
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/situp_resized.png} & 
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/squat_resized.png} & 
\includegraphics[width=0.16\linewidth]{drawings/dataset_imgs/lunge1.png} \\
(a) & (b) & (c) & (d) & (e) & (f) \vspace{-0.30cm}
\end{tabular}
\end{center}
\caption{{\small {\bf Success and Failure Cases, Meaningful splits:} (a-d) Training set samples. (e) A sample correctly labeled as normal. (f) A sample incorrectly labeled as normal. {\bf Top:} NTU-RGB+D split "???". {\bf Bottom}: Kinetics split "Pull Ups". The examples show the variety of actions grouped together within a meaningful split. Even though they take place in a similar setting, specific action poses can be siginificantly different. }
\label{fig:fail_cases}}
\end{figure}

==> drawings/tex/general_flow_fig.tex <==
\begin{figure} [!t]	
\begin{tabular}{c}
\includegraphics[width=0.94\linewidth]{drawings/pdf/general_flow.pdf} \vspace{0.0cm}
\end{tabular}
\caption{{\bf Suggested pipeline:} An input video is represented as a sequence of body poses. The sequences are embedded into latent space, and then soft-assigned into clusters. The soft-assignment vector serves as the representation of the input video. We use it jointly with a distribution learned during training phase as input for a normality scoring function. 
\lihi{What does the distribution capture?}
\amir{Need to draw sketch properly} }
\label{fig:general_flow}
\end{figure}        


==> drawings/tex/ntu_fvm_roc.tex <==
\begin{figure} [h!]  %[!h]

\begin{tabular}{c}
\includegraphics[width=0.96\linewidth]{result_figs/ntu/Mar05_0923_ntu_fvm_meaningful.pdf} \vspace{0.0cm}\\

\includegraphics[width=0.96\linewidth]{result_figs/ntu/Mar05_0923_ntu_fvm_rnd.pdf} \vspace{0.0cm}
\end{tabular}
\caption{{\bf Results for NTU-RGB+D dataset, Few-v-Many:} Average RoC curves for both split types: Top: Meaningful splits. Bottom: Random splits.  {\color{red} Todo: Choose color and dashing that make the graph readable in B\&W and in print} }

\label{plot:ntu_fvm}
\end{figure}        


==> drawings/tex/ntu_mvf_roc.tex <==
\begin{figure} [h!]  %[!h]

\begin{tabular}{c}
\includegraphics[width=0.94\linewidth]{result_figs/ntu/Mar05_0923_ntu_mvf_meaningful.pdf} \vspace{0.0cm}\\

\includegraphics[width=0.94\linewidth]{result_figs/ntu/Mar05_0923_ntu_mvf_rnd.pdf} \vspace{0.0cm}
\end{tabular}
\caption{{\bf Results for NTU-RGB+D dataset, Many-v-Few:} Average RoC curves for both split types: Top: Meaningful splits. Bottom: Random splits.   }

\label{plot:ntu_mvf}
\end{figure}        


==> supp_files/fail_cases_kin_para.tex <==
\section{Fail Cases - \emph{Kinetics-250}} \label{supp_kin_fail_cases}
Figure~\ref{fig:fail_cases} shows some failure cases. The recovered pose graph is super-imposed on the image. As can be seen, there is significant variability in scenes, viewpoints and poses of the people in what is considered a single ``normal'' data split. The two failures depicted show the weakness on relying solely on extracted pose for representing the action in a clip. We chose failure cases in which the pose is adequately extracted so we could focus on the model itself. 
% Clearly, a failure to extract poses would harm the method's results. 
% \amir{maybe move this failure cases to supp if we don't have enough space in the main body?}

Depicted in Figure~\ref{fig:fail_cases}, a ``lunge'' class clip which is to be considered normal is labeled abnormal when the instructor performs a single, slow and mostly static lunge throughout the clip, which we assume breaks the repetitive nature associated with lunge clips. The Second case, in which a standing-up Tai-chi instructor moves his hands forward and backward in a manner that may considered to be similar to a push ups arm movement, considered ``normal'' for that split.

% \input{drawings/tex/fail_cases_stc}
\input{drawings/tex/fail_cases_kin}


==> supp_files/kinetics_roc2.tex <==
\begin{figure*}
\begin{center}
\hspace*{-0.5cm}\begin{tabular}{@{\hskip 0.0cm}c@{\hskip -0.0cm}c@{\hskip -0.0cm}c@{\hskip -0.0cm}c@{\hskip 0.0cm}}
\includegraphics[width=0.41\linewidth]{result_figs/kinetics/Mar26_1059_kinetics_fvm_meaningful.pdf} & 
\includegraphics[width=0.41\linewidth]{result_figs/kinetics/Mar26_1059_kinetics_mvf_meaningful.pdf} & \vspace{-0.47cm} \\
\includegraphics[width=0.41\linewidth]{result_figs/kinetics/Mar26_1059_kinetics_fvm_rnd.pdf} &  
\includegraphics[width=0.41\linewidth]{result_figs/kinetics/Mar26_1059_kinetics_mvf_rnd.pdf}  \vspace{-0.12cm}\\
% \hspace{0.2cm}(a) & \hspace{0.2cm}(b) & \hspace{0.2cm}(c) & \hspace{0.2cm}(d) \vspace{-0.20cm}
\end{tabular}
\end{center}
\caption{{\small \textbf{Average ROC Curves for \textit{Kinetics-250} dataset.} \emph{``Sup.''} denotes the supervised baseline. Fill denotes standard deviation.}}
\label{plot:kinetics_roc}
\end{figure*}


==> supp_files/ntu_roc.tex <==
\begin{figure*}
\begin{center}
% \hspace*{-0.5cm}\begin{tabular}{@{\hskip 0.0cm}c@{\hskip -0.0cm}c@{\hskip -0.0cm}c@{\hskip -0.0cm}c@{\hskip 0.0cm}}
\hspace*{-0.5cm}\begin{tabular}{@{\hskip 0.0cm}c@{\hskip -0.0cm}c@{\hskip 0.0cm}}
\includegraphics[width=0.41\linewidth]{result_figs/ntu/Mar26_1100_ntu_fvm_meaningful.pdf} & 
\includegraphics[width=0.41\linewidth]{result_figs/ntu/Mar26_1100_ntu_mvf_meaningful.pdf} & \vspace{-0.55cm} \\
\includegraphics[width=0.41\linewidth]{result_figs/ntu/Mar26_1100_ntu_fvm_rnd.pdf} & 
\includegraphics[width=0.41\linewidth]{result_figs/ntu/Mar26_1100_ntu_mvf_rnd.pdf}  \vspace{-0.12cm}\\
\end{tabular}
\end{center}
\caption{{\small \textbf{Average ROC Curves for \textit{NTU-RGB-D} dataset.} \emph{``Sup.''} denotes the supervised baseline. Fill denotes standard deviation. }}
\label{plot:ntu_roc}
\end{figure*}

==> supp_files/roc_figs.tex <==
\section{Experiment Average ROC Curves}
The following figures depict the average ROC curves for each method for each of the settings. 

% \input{supp_files/ntu_roc.tex}
% \input{supp_files/kinetics_roc2.tex}

==> supp_files/supp_figs/basewords_coarse.tex <==

\begin{figure}
\begin{center}
\begin{tabular}{@{\hskip 0in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.06in}@{\hskip 0in}}
\includegraphics[width=0.3\linewidth]{supp_files/supp_figs/kin_clstr6_forecast_cropped.png} & 
\includegraphics[width=0.3\linewidth]{supp_files/supp_figs/kin_clstr7_armwrestling_cropped_resized.png} & 
\includegraphics[width=0.3\linewidth]{supp_files/supp_figs/kin_clstr10_crawling_cropped.png} \\

\multicolumn{1}{c}{(a)} & \multicolumn{1}{c}{(b)} & \multicolumn{1}{c}{(c)} \vspace{-0.25cm}\\

\end{tabular}
\end{center}
\caption{{\small \textbf{Base Words, \textit{Coarse-grained}:} 
Samples closest to cluster centroids, from a model trained on \emph{Kinetics-250} dataset, split \emph{Random6}. Frames from clips whose cluster assignment is closest to hard-assignment (one-hot), from three different clusters. 
Column (a) shows a sample from the 'presenting weather' class; 
Column (b) from the 'arm wrestling' class; and,
Column (c) from the 'crawling' class. 
Actions close to the centroids depict an essential manifestation of underlying action classes depicted. 
}}
\label{supp_basewords_coarse}
% \vspace{-0.2cm}
\end{figure}

==> supp_files/supp_figs/basewords_fine.tex <==
\begin{figure}
\begin{center}
\begin{tabular}{@{\hskip 0in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.06in}@{\hskip 0in}}
\includegraphics[width=0.3\linewidth]{supp_files/supp_figs/stc_clstr3_05_044_0756_cropped.jpg} & 
\includegraphics[width=0.3\linewidth]{supp_files/supp_figs/stc_clstr6_1_22_292_cropped.jpg} & 
\includegraphics[width=0.3\linewidth]{supp_files/supp_figs/stc_clstr7_02_004_900_cropped.jpg} \\

\multicolumn{1}{c}{(a)} & \multicolumn{1}{c}{(b)} & \multicolumn{1}{c}{(c)} \\ % \vspace{-0.15cm}\\

\end{tabular}
\end{center}
\caption{
{\small 
\textbf{Base Words, \textit{Fine-grained}:} 
Samples closest to cluster centroids, from a model trained on \emph{ShanghaiTech} dataset. Frames from clips whose cluster assignment is closest to hard-assignment (one-hot), from three different clusters. 
Column (a) depicts a person walking towards the camera;
Column (b) depicts a person walking across the frame, perpendicular to the camera (person closer to camera); and,
Column (c) depicts a person walking away and across from the camera, in a $45^{\circ}$ angle (person to the right).
Actions close to the centroids depict a common variation of the action in hand, in this case, the walking direction.
} % \small
} % \caption
\label{supp_basewords_fine}
% \vspace{-0.2cm}
\end{figure}

==> tables/noise_ablation_table.tex <==
\begin{table}
\centering
% \begin{center}
\begin{tabular}{l c c c c c} % \hspace*{} for Left-right shift of the entire table
\toprule
\textbf{Method} & \textbf{0.1} & \textbf{1.0} & \textbf{5.0} & \textbf{10.0} & \textbf{20.0} \\
\midrule            
Few vs. Many   & 0.?? & 0.?? & 0.?? \\ 
Many vs. Few  & 0.?? & \bf{0.??} & 0.?? \\
\bottomrule
\end{tabular}
% \end{center}
\vspace{0.1cm}		
\caption{ \small{\bf Robustness to Noise:} Results for {\it NTU-RGB+D} Few vs.\ Many Experiment, split "Music": \amir{Perhaps turn into a graph}}
\label{tables:noise_ablation}
% \vspace{-0.1cm}
\end{table}	
